A Survey on Masked Autoencoder for Self-supervised Learning in Vision and Beyond

Masked autoencoders are scalable vision learners, as the title of MAE \cite{he2022masked}, which suggests that self-supervised learning (SSL) in vision might undertake a similar trajectory as in NLP. Specifically, generative pretext tasks with the masked prediction (e.g., BERT) have become a de facto standard SSL practice in NLP. By contrast, early attempts at generative methods in vision have been buried by their discriminative counterparts (like contrastive learning); however, the success of mask image modeling has revived the masking autoencoder (often termed denoising autoencoder in the past). As a milestone to bridge the gap with BERT in NLP, masked autoencoder has attracted unprecedented attention for SSL in vision and beyond. This work conducts a comprehensive survey of masked autoencoders to shed insight on a promising direction of SSL. As the first to review SSL with masked autoencoders, this work focuses on its application in vision by discussing its historical developments, recent progress, and implications for diverse applications.

==> tab/ablations.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
Method & Frobnability & Frobnability & Frobnability \\
\midrule
Ours v0 & Frumpy \\
Ours v1 & Frobbly \\
\textbf{Ours} & Makes one's heart Frob\\
\bottomrule
\end{tabular}
} %< \resizebox
\caption{
% 
\textbf{Ablations} -- our decisions are well justified.
% 
} % \caption
\label{tab:ablations}
\end{table}

==> tab/epoch_bs_dataset.tex <==
\begin{table}
    \centering
    % \resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
    \begin{tabular}{@{}cccc@{}}
    \toprule
    % \textbf{Method} & 
    Batch Size & SimCLR (\%) & DT(\%) & Improvement ($\Delta$) \\
    \midrule
    % \multirow{7}{*}{SimCLR}
    16 & 38.89 & 40.49 & \textbf{+ 1.6} \\
    32 & 46.79 & 51.78 & \textbf{+ 5.0} \\
    64 & 53.06 & 57.49 & \textbf{+ 4.4}\\
    128 & 55.75 & 60.30 & \textbf{+ 4.6} \\
    256 & 56.41 & 59.38 & \textbf{+ 3.0} \\
    512 & 57.13 & 59.12 & \textbf{+ 2.0} \\
    1024 & 56.93 & 57.36 & \textbf{+ 0.4} \\
    % \midrule
    % \multirow{6}{*}{DT}
    % & 16 & - \\
    % & 32 & - \\
    % & 64 & 57.49 \\
    % & 128 & 60.30 \\
    % & 256 & 59.38 \\
    % & 512 & 59.12 \\
    % & 1024 & 57.36 \\
    \bottomrule
    \end{tabular}
    % } % \resizeboxs
    \caption{
    % 
    The comparision of our method Dual Temperature (DT) and baseline SimCLR. In Cifar 100, using ResNet-18, epoch 250. SimCLR temperature 0.1. our Dual Temperature $\tau_{intra} = 0.1, \tau_{inter} = 1$.
    %\textbf{State of the art} -- Glory to the bold numbers.
    % 
    } % \caption
    \label{tab:sota1}
\end{table}


==> tab/sota.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
Method & Frobnability & Frobnability & Frobnability \\
\midrule
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\bottomrule
\end{tabular}
} % \resizebox
\caption{
% 
\textbf{State of the art} -- Glory to the bold numbers.
% 
} % \caption
\label{tab:sota}
\end{table}
